ActiveCheerios: 3D-Printed Marangoni-Driven Active Particles at an Interface

Marangoni surfers are simple, cost-effective tabletop experiments that, despite their simplicity, exhibit rich dynamics and collective behaviors driven by physicochemical mechanisms, hydrodynamic interactions, and inertial motion. This work introduces self-propelled particles designed and manufactured through 3D printing to move on the air-water interface. We develop particles with tunable motility and controlled particle-particle interactions by leveraging surface tension-mediated forces, such as the Marangoni effect for propulsion and the Cheerios effect for interactions. Rapid prototyping through 3D printing facilitates the exploration of a wide design space, enabling precise control over particle shape and function. We exemplify this by creating translational and chiral particles. Additionally, we investigate self-assembly in this system and highlight its potential for modular designs where mechanically linked particles with varying characteristics follow outlined trajectories. This research offers a flexible, low-cost approach to designing active interfacial systems and opens new possibilities for further advancements of adaptive, multifunctional devices.

==> colors_define.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\definecolor{darkorange}{rgb}{1.0, 0.55, 0.0}
\definecolor{persiangreen}{rgb}{0.0, 0.65, 0.58}
\definecolor{persianindigo}{rgb}{0.2, 0.07, 0.48}
\definecolor{cadet}{rgb}{0.33, 0.41, 0.47}
\definecolor{turquoisegreen}{rgb}{0.63, 0.84, 0.71}
\definecolor{sandybrown}{rgb}{0.96, 0.64, 0.38}
\definecolor{blueblue}{rgb}{0.0, 0.2, 0.6}
\definecolor{ballblue}{rgb}{0.13, 0.67, 0.8}
\definecolor{greengreen}{rgb}{0.0, 0.5, 0.0}
